Hazy blue worlds: A holistic aerosol model for Uranus and Neptune, including Dark Spots

We present a reanalysis (using the Minnaert limb-darkening approximation) of visible/near-infrared (0.3 - 2.5 micron) observations of Uranus and Neptune made by several instruments. We find a common model of the vertical aerosol distribution that is consistent with the observed reflectivity spectra of both planets, consisting of: 1) a deep aerosol layer with a base pressure > 5-7 bar, assumed to be composed of a mixture of H2S ice and photochemical haze; 2) a layer of photochemical haze/ice, coincident with a layer of high static stability at the methane condensation level at 1-2 bar; and 3) an extended layer of photochemical haze, likely mostly of the same composition as the 1-2-bar layer, extending from this level up through to the stratosphere, where the photochemical haze particles are thought to be produced. For Neptune, we find that we also need to add a thin layer of micron-sized methane ice particles at ~0.2 bar to explain the enhanced reflection at longer methane-absorbing wavelengths. We suggest that methane condensing onto the haze particles at the base of the 1-2-bar aerosol layer forms ice/haze particles that grow very quickly to large size and immediately 'snow out' (as predicted by Carlson et al. 1988), re-evaporating at deeper levels to release their core haze particles to act as condensation nuclei for H2S ice formation. In addition, we find that the spectral characteristics of 'dark spots', such as the Voyager-2/ISS Great Dark Spot and the HST/WFC3 NDS-2018, are well modelled by a darkening or possibly clearing of the deep aerosol layer only.

==> README <==

TrackChanges
Multiple editors in LaTeX.
========================================================================

INTRODUCTION:

  The TrackChanges package consists of two parts:
  1.  A LaTex style file: 
        trackchanges.sty
  2.  A GUI, written in python:
         trackchanges.py

  The style file may be used without the GUI.  The GUI is to be used to
  facilitate accepting, rejecting, or modifying the edits made using the
  commands defined in the style file.

  This packages also includes a command line utility: acceptchanges.py.
  This utility will only work in posix environments.

  Help files are available as part of this package:
    ./documentation/web/help.html

  Documentation is also  available at the TrackChanges website.

  To get the latest version of this sofware go to:
    http://trackchanges.sourceforge.net

========================================================================

LaTeX STYLEFILE:

  INSTALLATION:
    Copy the style file to the directory with your LaTeX document.
    The style file can be found at: ./LatexPackage/trackchanges.sty

  USAGE:
    Add the following line to you latex document:
      \usepackage{trackchanges}

    Add the names of the editors in the preamble [OPTIONAL]:
      \addeditor{editor}

    Now you have access to all of the TrackChanges commands:
      \add[editor]{added text}
      \remove[editor]{removed text}
      \change[editor]{removed text}{added text}
      \note[editor]{note text}
      \annote[editor]{text to annotate}{note text}

    See the documentation or website for display options.

========================================================================

TRACKCHANGES GUI

  This is a Beta version of the TrackChanges GUI. 
  That means: Beware! Bugs may lurk ahead.

  If you choose to use this software plese be careful to back up your 
  TeX files.  This software has not been thoroughly tested and may
  corrupt your TeX files.  (The style file is fine and can't mess any
  thing up but the GUI for accepting/rejecting/modifying might.)

  ----------------------------------------------------------------------
  
  WARNING:  
    This program has not be generalized to handle international
    characters.  Such characters may cause unexpected behavior.
  
  NOTE:
    So far the GUI has only been tested on Windows XP and Os X.
    While it should work on linux, it might not.
  
  WARNING (AGAIN):
    This is beta software. It has not been tested much.
    Things may be broken.
  
  
  
  ----------------------------------------------------------------------
  INSTALLATION:
    Once you have all the dependencies installed, 
    just run ./PythonPackage/trackchanges.py
    
      $> cd PythonPackage
      $> python trackchanges.py
  
  
  ----------------------------------------------------------------------
  DEPENDANCIES:
    To get the trackchanges GUI to run you will need several things:
     
    1. Python 2.6 or later
    2. PyQt 4.4.4 or later
  
  ----------------------------------------------------------------------
  WHERE TO GET DEPENDANCIES:
    Python 2.6  -- http://www.python.org/
    PyQt 4      -- http://www.riverbankcomputing.co.uk/
  
  


========================================================================

This file is part of TrackChanges
Copyright 2009 Novimir Antoniuk Pablant
               Felix Salfner

TrackChanges is free software: you can redistribute it and/or modify
it under the terms of the GNU General Public License as published by
the Free Software Foundation, either version 2 of the License, or
(at your option) any later version.

TrackChanges is distributed in the hope that it will be useful,
but WITHOUT ANY WARRANTY; without even the implied warranty of
MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
GNU General Public License for more details.

You should have received a copy of the GNU General Public License
along with TrackChanges.  If not, see <http://www.gnu.org/licenses/>.

------------------------------------------------------------------------
